Curvas de contato no espa\c{c}o projetivo

The odd dimensional projective space $\mathbb{P}^{2n-1}$ admits a contact structure arising from a non integrable distribution of hyperplanes determined by a symplectic form in $\mathbb{C}^{2n}$. Our object of interest is the set of rational curves of degree d which are tangent to that contact distribution in $\mathbb{P}^3$. Such curves are called contact curves or legendrian curves. To explore the geometry of contact curves, we construct the parameter space $\mathcal{L}_d$ using Kontsevich's stable maps, $\overline{\mathcal{M}}_{0,0}(\mathbb{P}^3,d)$, endowed with the structure of algebraic stack. The intersection theory on stacks allows us to define in that space the virtual invariant $N_d$, associated with the number of degree $d$ contact curves incident to $2d+1$ lines. Using graph combinatorics and partitions originated from Bott's localization formula, we determine a general formula for $N_d$. We explicitly calculate it for contact curves up to degree 4 - confirming the known cases of contact lines and conics and introducing the new numbers for cubics and quartics. Finally, we discuss the enumerative significance of these invariants, still conjectural for $d>4$.

==> ContactStructure.tex <==
\newpage

\section{Estrutura de contato}\label{SS}  %sympletic structure

\p Nessa seção definimos nosso principal objeto de estudo: curvas de contato. Essas curvas aparecem em espaços de dimensão ímpar com a chamada estrutura de contato, proveniente da um espaço simplético. Os conceitos e nomenclaturas para as estruturas simplética e de contato são apresentados em (\ref{CC.symp}), tendo como referência básica o texto \cite{Dynamical}.

\subsection{A estrutura simplética}\label{CS.sympletic}

\p Em um espaço vetorial complexo $V$, dizemos que uma 2-forma $\omega:V \times V \rightarrow \C$ é \textbf{simplética} se
\begin{itemize}
\item é bilinear: $\omega(\alpha u + v,w)=\alpha\omega(u,w) + \omega(v,w)$
\item é anti-simétrica: $\omega(v,w) = -\omega(w,v)$
\item é não degenerada: para todo $v$, existe $w$ tal que $\omega(v,w) \neq 0$
\end{itemize}

Observe que se um espaço vetorial possui forma simplética, ele deve ter dimensão par. Portanto, consideremos daqui em diante o espaço $V=\C^{2r}$, $r$ inteiro. Se tomamos em $\C^{2r}$ coordenadas $x=(x_1,\cdots,x_r,y_1,\cdots,y_r)$, uma 2-forma simplética, única a menos de uma mudança de coordenadas simpléticas, é 
$$
\omega=\sum_{i=1}^{r}dx_i \wedge dy_i.
$$

Um espaço vetorial munido de uma forma simplética é chamado \textbf{espaço simplético}. Dado um subespaço linear $W$, definimos o seu complementar relativo à forma $\omega$ por
$$
W^{\perp} = \{ v \in \C^{2r} \tq \omega(w,v)=0 \; \forall w \in W \}.
$$
Claramente, temos as relações $(W^{\perp})^{\perp}= W$ e $\dim W + \dim W^{\perp} = 2r$. Do fato dessa forma ser simplética, podemos ainda definir alguns subespaços especiais:
\begin{itemize}
\item $W$ é simplético se $W \cap W^{\perp} = \{0\}$
\item $W$ é isotrópico se $W \subseteq W^{\perp}$
\item $W$ é coisotrópico se $W^{\perp} \subseteq W$, ou se $W^{\perp}$ é isotrópico.
\item $W$ é Lagrangiano se $W^{\perp} = W$, ou $W$ é isotrópico e coisotrópico.
\end{itemize} 

Observe que se $W$ é isotrópico, temos $\dim W \le r$; se é coisotrópico, $\dim W \ge r$. Em particular, se $W$ é Lagrangiano, $\dim W = r$. Outro modo de dizer: $W$ é Lagrangiano se é um subespaço maximal tal que $\omega|_W \equiv 0$.

Também temos uma classificação das variedades em um espaço simplético: uma subvariedade é chamada isotrópica, coisotrópica ou Lagrangeana se os são seus espaços tangentes em cada ponto não singular.

\subsection{A distribuição de contato}\label{CS.contact}

\p Apesar da estrutura simplética estar definida somente em um espaço vetorial de dimensão par, temos uma estrutura análoga para um espaço projetivo de dimensão ímpar. De fato, $\P^{2r-1} = \P(\C^{2r})$ herda certas propriedades da estrutura simplética do espaço linear associado. Vamos descrever melhor essa estrutura.  

Dado um espaço simplético $(\C^{2r},\omega)$, temos o isomorfismo
$$
\begin{array}{rcl}
\C^{2r} & \rightarrow & (\C^{2r})^{\vee} \\
v & \mapsto & \omega(v,\cdot)
\end{array}
$$

Assim, para cada ponto $p \in \P^{2r-1}$, consideramos uma forma diferencial que sobre o ponto $p$ é $\omega_p := \omega(p,\cdot)$, definida a menos de múltiplo escalar. Também denotaremos essa forma por $\omega$. Essa forma diferencial define uma distribuição de hiperplanos em $T\P^{2r-1}$ determinados por $p \mapsto \Nuc \omega_p$. Observe que $\omega_p(p)=0$, pois $\omega$ é alternada, o que nos permite realizar $\omega$ como uma distribuição de hiperplanos em $\P^{2r-1}$. Vale também que $\omega \wedge (d\omega)^{\wedge r-1}$ é não degenerada, característica também tida como uma `não integrabilidade maximal'. A essa distribuição damos o nome de \textbf{distribuição de contato} e dizemos que a forma $\omega$ com $\omega \wedge (d\omega)^{\wedge r-1}$ não degenerada define uma \textbf{estrutura de contato} em $\P^{2r-1}$.

Estamos interessados em analisar a condição de tangência à essa distribuição.

\begin{defi}\label{d.contact.curve}
Seja $X$ uma subvariedade de $\P^{2r-1}$ com sua estrutura de contato $\omega$. Dizemos que $X$ é uma \textbf{subvariedade de contato} se é tangente à distruibuição de contato em cada um de seus pontos não singulares. Isto é, se
 $$
 T_pX \subset \Nuc \omega_p, \; \forall p \in X \setminus Sing\, X
 $$
\end{defi}

Observe que para uma subvariedade de contato, temos $\omega \wedge d\omega_p =0$. \textcolor[rgb]{1,0,0}{[comentários]}. De fato, $d\omega_p$ dá uma estrutura simplética ao hiperplano $\Nuc\omega_p$, no qual $T_pX$ é então um subespaço isotrópico. De outra forma, o cone afim da subvariedade $X$, $C(X) \subset \C^{2r}$, deve ser uma subariedade isotrópica. Dessa forma, a dimensão de uma subvariedade de contato deve ser no máximo $r-1$. 

Outras definições: dizemos que uma variedade $X \in \P^{2r-1}$ é \textbf{involutiva} se seu cone afim em $\C^{2r}$ é coisotrópico. Se $X$ é involutiva com $\dim X = r-1$, ou $C(X)$ é Lagrangiano, dizemos que $X$ é \textbf{Legendriana}.

Em particular - e na verdade nosso caso de interesse - uma curva de contato em $\P^3$ é Legendriana (ge portanto, também involutiva). 

